Natural orbitals and sparsity of quantum mutual information

Natural orbitals, defined in electronic structure and quantum chemistry as the (molecular) orbitals diagonalizing the one-particle reduced density matrix of the ground state, have been conjectured for decades to be the perfect reference orbitals to describe electron correlation. In the present work we applied the Wavefunction-Adapted Hamiltonian Through Orbital Rotation (WAHTOR) method to study correlated empirical ans\"atze for quantum computing. In all representative molecules considered, we show that the converged orbitals are coinciding with natural orbitals. Interestingly, the resulting quantum mutual information matrix built on such orbitals is also maximally sparse, providing a clear picture that such orbital choice is indeed able to provide the optimal basis to describe electron correlation. The correlation is therefore encoded in a smaller number of qubit pairs contributing to the quantum mutual information matrix.

==> algorithm.tex <==
\section{IMPROVED WAHTOR ALGORITHM}
\label{algorithm}
In this section, we illustrate how we modified the WAHTOR algorithm in order to reduce the computational cost due to the repetition of a considerable number of VQEs. Remember that the WAHTOR method optimises both the wave function parameters and the rotation parameters of the Hamiltonian.
While the ansatz $\ket{\Psi(\bm{\theta})}$ is parameterized by the values of the components of the vector $\bm{\theta}$, the basis changes of the system can be represented with the following unitary matrices: 
\begin{equation}
U(\bm{R})=e^{i\bm{R}\cdot\bm{T}}
\label{eq:U}
\end{equation}
where $\bm{T}$ are the generators of the Lie group and $\bm{R}$ is a vector of real components that represent the parameters of the unitary transformation applied to the Hamiltonian. The second quantized molecular Hamiltonian in a generic basis set, dependent on the $\bm{R}$ parameters, is written as:
\begin{equation}
H(\bm{R})=\sum_{i,j}h(\bm{R})_{ij}a^\dag_i a_j+\frac{1}{2}\sum_{c,d,e,f}h(\bm{R})_{cdef}a^\dag_c a^\dag_d a_e a_f 
\label{eq:molH}
\end{equation}
where $a^\dag$ and $a$ are respectively the creation and the annihilation operators acting on the specific molecular orbital identified by the $i,j,c,d,e,f$ indices. $h_{ij}(\bm{R})$ and $h_{cdef}(\bm{R})$ are respectively the components of the one and two body integrals in the molecular basis set determined by the parameter $\bm{R}$. Since the Hatree-Fock molecular basis set is associated to $\bm{R}=0$, the two and four indices tensors defined above can be obtained from the Hatree-Fock ones, $h_{1_{HF}}$ and $h_{2_{HF}}$, by the following equations:
\begin{equation}
h_1(\bm{R})=e^{i\bm{R}\cdot\bm{T}}h_{1_{HF}}e^{-i\bm{R}\cdot\bm{T}}
\end{equation} 
and
\begin{equation}
h_2(\bm{R})=e^{i\bm{R}\cdot\bm{T}}\otimes e^{i\bm{R}\cdot\bm{T}}h_{2_{HF}}e^{-i\bm{R}\cdot\bm{T}}\otimes e^{-i\bm{R}\cdot\bm{T}}
\end{equation}
The energy cost function
\begin{equation}
E(\bm{R},\bm{\theta})=\bra{\Psi(\bm{\theta})}H(\bm{R})\ket{\Psi(\bm{\theta})}
\label{eq:energy}
\end{equation}
depends on both set of parameters $\bm{\theta}$ and $\bm{R}$.
Since the adiabatic WAHTOR algorithm is based on the steepest descent optimiser, a VQE is carried out for each step of the Hamiltonian optimisation, thus for each calculation of the energy derivative. The improvement we propose makes it possible to reduce the number of VQEs performed using higher-order optimisers.
Energy can be optimized with respect to $\bm{R}$ parameters by calculating its n-order analytical derivatives:
\begin{equation}
\begin{split}
\frac{d^n E(\bm{R})}{d \bm{R}^n}=\sum_{i,j}\frac{d^n h(\bm{R})_{ij}}{d \bm{R}^n}\bra{\Psi(\bm{\theta})}a^\dag_i a_j\ket{\Psi(\bm{\theta})}+ \\
+\frac{1}{2}\sum_{c,d,e,f}\frac{d^n h(\bm{R})_{cdef}}{d \bm{R}^n}\bra{\Psi(\bm{\theta})}a^\dag_c a^\dag_d a_e a_f\ket{\Psi(\bm{\theta})}
\end{split}
\label{eq:dH}
\end{equation}
from which one can see the dependence on the n-order derivatives of the one and two body integrals. In particular, in order to implement a trust region optimizer, we are interested in the first and the second derivatives of the integrals in $\bm{R}=\bm{0}$:
\begin{equation}
\begin{split}
& \frac{dh_1(\bm{R})}{dR_l}|_{\bm{R}=\bm{0}}=i[T_{l},h_{1_{HF}}] \\
& \frac{d h_2(\bm{R})}{dR_l}|_{\bm{R}=\bm{0}}=i[T_l\otimes I+I\otimes T_l,h_{2_{HF}}]
\end{split}
\end{equation}
and 
\begin{equation}
\begin{split}
&\frac{d^2 h_1(\bm{R})}{dR_{l_1}dR_{l_2}}|_{\bm{R}=\bm{0}}=-\frac{1}{2}([T_{l_1},[T_{l_2},h_{1_{HF}}]]+ \\
& +[T_{l_2},[T_{l_1},h_{1_{HF}}]]) \\
&\frac{d^2 h_2(\bm{R})}{dR_{l_1}dR_{l_2}}|_{\bm{R}=\bm{0}}=-\frac{1}{2}([T_{l_1}\otimes I+I\otimes T_{l_1},[T_{l_2}\otimes I+ \\
& +I\otimes T_{l_2},h_{2_{HF}}]]+[T_{l_2}\otimes I+I\otimes T_{l_2},[T_{l_1}\otimes I+ \\
& +I\otimes T_{l_1},h_{2_{HF}}]])
\end{split}
\end{equation}
where $I$ is the identity operator. The proofs of these equations can be found in the supplementary material. 
\begin{figure}
\includegraphics[width=0.95\linewidth]{grafici/algorithm.pdf}
\caption{The scheme of the non-adiabatic WAHTOR algorithm is defined in this article.}
\label{fig:scheme}
\end{figure}
The improved WAHTOR is based on the alternation of wave function optimisation, i.e. the execution of a VQE, and Hamiltonian optimisation. More specifically, in this case, once it has been defined the initial Hamiltonian in the Hartree Fock basis, we apply the rotation operator for the basis change,
resulting in a new $\bm{R}$-dependent Hamiltonian. Keeping the rotation parameters fixed, we perform a VQE algorithm for the optimisation of the wave function.
Once the optimisation of $\bm{\theta}$ is concluded, we perform the Hamiltonian optimization. In this way, the Hamiltonian and the ansatz parameters are alternatively optimized until convergence is reached. This new scheme, represented in figure \ref{fig:scheme}, is named non-adiabatic WAHTOR.  
Using this method, we do not calculate the derivatives between two VQE runs, as in the case of the adiabatic WAHTOR \cite{}, but we optimise the rotation parameters between the two VQEs. The result is faster optimisation and fewer VQEs: the expectation value of the Pauli strings that appear in equation \ref{eq:dH} do not change during the Hamiltonian optimization step and their value is obtained in the step of the previous VQE. 
If we need to calculate the expectation value of a new Pauli string for the evaluation of the derivatives, we do it once and save this value until the end of the optimization. With respect to the adiabatic algorithm, the non adiabatic one reduces the number of times that the VQE runs, so the computation cost for the QPU.   

==> computational_details_old.tex <==
\section{COMPUTATIONAL DETAILS}
\label{computational_details_old}

{\it \textbf{Improved WAHTOR algorithm}}\\
(qui ci metterei solo un riassuntino di WAHTOR)\\
\textcolor{red}{da scrivere}

{\it \textbf{Simulated systems}}\\
We considered seven different molecular systems: $H_2$, $LiH$, $HF$, $BeH_2$, $H_2O$, $H_2S$, and $NH_3$. Depending on the systems we used different basis sets and frozen core approximations, as detailed by table \ref{table_molecule_info}.
\begin{table*}[hb!]
\caption{Geometric distances, basis set, number of qubits of each molecule under investigation.}
\label{table_molecule_info}
\centering
\newcommand{\minitab}[2][l]{\begin{tabular}#1 #2\end{tabular}}
\begin{tabular}{| c | c | c | c |}
\hline
\hline 
molecule &  atomic positions (\AA{}) &  basis set &  qubits \\ 
\hline
\hline
$H_2$   & \minitab[c]{H 0.0 0.0 0.0 \\ H 0.0 0.0 0.74}  & 6-31g  & 8 \\
\hline
$LiH$   & \minitab[c]{Li 0.0 0.0 0.0 \\ H 0.0 0.0 1.595}  & sto-3g  & 10  \\
\hline
$HF$    & \minitab[c]{F 0.0 0.0 0.0 \\ H 0.0 0.0 0.917}  & sto-3g  & 10  \\
\hline 
$BeH_2$ & \minitab[c]{H 0.0 0.0 0.0 \\ Be 0.0 0.0 1.334 \\ H 0.0 0.0 2.668}  & sto-3g  & 12 \\
\hline 
$H_2O$  & \minitab[c]{O 0.0 0.0 0.0 \\ H 0.757 0.586 0.0 \\ H -0.757 0.586 0.0}
& sto-3g  & 12 \\
\hline
$H_2S$  & \minitab[c]{S 0.0 0.0 0.0 \\ H 0.0 0.9616 -0.9269 \\ H 0.0 -0.9616 -0.9269}  & sto-3g  & 12  \\
\hline        
$NH_3$  & \minitab[c]{N 0.0 0.0 0.1211 \\ H 0.0 0.9306 -0.2826 \\ H 0.8059 -0.4653 -0.2826	\\ H -0.8059 -0.4653 -0.2826}  & sto-3g  & 14  \\
\hline		
\end{tabular}
\end{table*}
We use the Jordan-Wigner encoding method \cite{Jordan1928} obtaining a number of qubits ranging from 8 to 14. The Hartree-Fock orbitals and the terms of the molecular Hamiltonian have been obtained using the PySCF Python package. \cite{pyscf} The WAHTOR algorithm has been implemented by a in-house produced Python program exploiting the Qiskit Python libraries. \cite{qiskit}

The variational energies results obtained using VQE and WAHTOR algorithms
percentage of correlation energy is reported as  defined by
\begin{equation}
E_{corr}=\frac{E_{calculated}-E_{HF}}{E_{full-CI}-E_{HF}}
\end{equation}
where $E_{full-CI}$ is the exact energy, $E_{calculated}$ is the energy calculated using VQE or WAHTOR algorithm and $E_{HF}$ is the Hartree-Fock energy.

{\bf A questo punto farei due tabelle, una con i sistemi ed i qubits e l'altra con i risultati. E' più logico. Ognuna prende una colonna} \\

Table \ref{table_molecule}, in addition to showing the energy results obtained, provides the value of the dimensionless parameter $\delta\in [0,1]$ that measures how much the converged WAHTOR orbitals ($\ket{W}$) are close to the natural ones ($\ket{NO}$), calculated from the exact Full-CI state.

\begin{equation}
\delta=\frac{\sum_i(|\braket{W_i|NO_i}|-|\braket{HF_i|NO_i}|}{N-\sum_i|\braket{HF_i|NO_i}|}
\end{equation}
where $N$ is the number of orbitals considered and $\ket{HF}$ are the Hartree-Fock ones. So the closer the $\delta$ value is to 1, the more the optimized orbitals are similar to the reference natural orbitals (corresponding to $\delta=1$); the closer it is to zero, the more the optimized orbitals are closer to the Hartree Fock orbitals (corresponding to $\delta=0$).
\\
\begin{figure}[h]
\centering
\begin{equation}
    \Qcircuit @C=0.7em @R=0.3em {
   	    	& \lstick{\ket{0}} & \gate{R_y(\theta_0)} & \ctrl{1} & \qw & \qw & \qw & \qw & \qw & \qw & \gate{R_y(\theta_8)} & \qw &\\
   	    	& \lstick{\ket{1}} & \gate{R_y(\theta_1)} & \targ & \ctrl{1} & \qw & \qw & \qw & \qw & \qw & \gate{R_y(\theta_9)} & \qw &\\
   	    	& \lstick{\ket{2}} & \gate{R_y(\theta_2)} & \qw & \targ & \ctrl{1} & \qw & \qw & \qw & \qw & \gate{R_y(\theta_{10})} &\qw &\\
   	    	& \lstick{\ket{3}} & \gate{R_y(\theta_3)} & \qw & \qw & \targ & \ctrl{1} & \qw & \qw & \qw & \gate{R_y(\theta_{11})} & \qw &\\
   	    	& \lstick{\ket{4}} & \gate{R_y(\theta_4)} & \qw & \qw & \qw & \targ & \ctrl{1} & \qw & \qw & \gate{R_y(\theta_{12})} &\qw & \\
   	    	& \lstick{\ket{5}} & \gate{R_y(\theta_5)} & \qw & \qw & \qw & \qw & \targ & \ctrl{1} & \qw & \gate{R_y(\theta_{13})} & \qw & \\
   	    	& \lstick{\ket{6}} & \gate{R_y(\theta_6)} & \qw & \qw & \qw & \qw & \qw & \targ & \ctrl{1} & \gate{R_y(\theta_{14})} & \qw &\\
   	    	& \lstick{\ket{7}} & \gate{R_y(\theta_7)} & \qw & \qw & \qw & \qw & \qw & \qw & \targ & \gate{R_y(\theta_{15})} & \qw & \\
   	    	\ar@{-}[]+<5.3em,15.8em>;[]+<5.3em,-0.0em>
   	    	\ar@{-}[]+<5.4em,15.8em>;[]+<5.4em,-0.0em>
   		    \ar@{-}[]+<20.5em,15.8em>;[]+<20.5em,-0.0em>
   		    \ar@{-}[]+<20.6em,15.8em>;[]+<20.6em,-0.0em>
        }
\notag
\end{equation}
\caption{Ladder entangler map for an 8-qubits system. The quantum gates between the two barriers compose the block (identified by bold lines in the figure). Each block is repeated a certain number of times $d$, which is defined as the depth of the circuit.}
\label{fig:ansatz_example}
\end{figure}

\begin{table*}[]
\caption{Basis set, number of qubits, VQE and WAHTOR percentage correlation energy results and geometric distance from the reference natural orbitals for each molecule under investigation.}
\label{table_molecule}
\centering
\newcommand{\minitab}[2][l]{\begin{tabular}#1 #2\end{tabular}}
\begin{tabular}{| c | c | c | c |}
\hline
\hline 
molecule &  \% VQE & \% WAHTOR &  $\delta$\\ 
\hline
\hline
$H_2$ & 47.08  & 98.05  & 0.998  \\
\hline
$LiH$ & 72.14  & 94.75  & 0.999  \\
\hline
$HF$ & 71.51  & 93.03  & 0.999  \\
\hline 
$BeH_2$ & 45.40  & 45.42  & $\ket{HF}\equiv\ket{NO}$  \\
\hline 
$H_2O$ & 51.65  & 73.54  & 0.972  \\
\hline
$H_2S$ & 74.76  & 87.42  & 0.998  \\
\hline        
$NH_3$ & 36.42  & 41.85  & 0.988\\
\hline		
\end{tabular}
\end{table*}


\iffalse
\begin{table*}[]
\caption{Basis set, number of qubits, VQE and WAHTOR percentage correlation energy results and geometric distance from the reference natural orbitals for each molecule under investigation.}
\label{table_molecule}
\centering
\newcommand{\minitab}[2][l]{\begin{tabular}#1 #2\end{tabular}}
\begin{tabular}{c | c | c | c | c | c | c}
\hline
\hline 
molecule &  atomic positions (\AA{}) &  basis set &  qubits & \% VQE & \% WAHTOR &  $\delta$\\ 
\hline
\hline
$H_2$   & \minitab[c]{H 0.0 0.0 0.0 \\ H 0.0 0.0 0.74}  & 6-31g  & 8  & 47.08  & 98.05  & 0.998  \\
\hline
$LiH$   & \minitab[c]{Li 0.0 0.0 0.0 \\ H 0.0 0.0 1.595}  & sto-3g  & 10  & 72.14  & 94.75  & 0.999  \\
\hline
$HF$    & \minitab[c]{F 0.0 0.0 0.0 \\ H 0.0 0.0 0.917}  & sto-3g  & 10  & 71.51  & 93.03  & 0.999  \\
\hline 
$BeH_2$ & \minitab[c]{H 0.0 0.0 0.0 \\ Be 0.0 0.0 1.334 \\ H 0.0 0.0 2.668}  & sto-3g  & 12  & 45.40  & 45.42  & $\ket{HF}\equiv\ket{NO}$  \\
\hline 
$H_2O$  & \minitab[c]{O 0.0 0.0 0.0 \\ H 0.757 0.586 0.0 \\ H -0.757 0.586 0.0}
& sto-3g  & 12  & 51.65  & 73.54  & 0.972  \\
\hline
$H_2S$  & \minitab[c]{S 0.0 0.0 0.0 \\ H 0.0 0.9616 -0.9269 \\ H 0.0 -0.9616 -0.9269}  & sto-3g  & 12  & 74.76  & 87.42  & 0.998  \\
\hline        
$NH_3$  & \minitab[c]{N 0.0 0.0 0.1211 \\ H 0.0 0.9306 -0.2826 \\ H 0.8059 -0.4653 -0.2826	\\ H -0.8059 -0.4653 -0.2826}  & sto-3g  & 14  & 36.42  & 41.85  & 0.988\\
\hline		
\end{tabular}
\end{table*}
\fi

{\it \textbf{Implementation of quantum algorithm}}\\
The parametrized quantum circuit chosen in the present work belongs to the so-called heuristic ansatzes build as following. Firstly, a repetition of single qubit rotations around the y-axis is applied to the n-qubits Hartree−Fock reference state. After such rotations, an entangling block composed of CNOT gates followed by another set of independent rotations on each qubit has been applied. The block composed by CNOT gates and rotations can be therefore repeated a certain number of times, each time using different variational parameters, as shown in figure \ref{fig:ansatz_example}. The total number of blocks determines the circuit depth. In this work, we considered depth 2 for diatomic molecules and depth 4 for molecules composed of 3 or 4 atoms. CNOT gates are arranged to form a ladder, as shown in figure \ref{fig:ansatz_example} for each molecule considered here except for $NH_3$, for which we considered an ansatz topology with less than 13 CNOT gates. For each molecular system we execute 100 VQE runs for starting from different variational parameters and the lowest energy result was considered as starting point for the WAHTOR algorithm. We optimized the ansatz parameters using the L-BFGS-B optimizer.\cite{Byrd1995}
The convergence is reached when in two successive WAHTOR iteration the VQE energies differ less than $10^{-6}$ Hartree. All  simulations are executed using the statevector simulator. 
\\

{\it \textbf{Implementation of derivatives}}\\
For the implementation of the WAHTOR algorithm, the matrices that determine the basis change take spin symmetry into account, i.e. the spin-up and the spin-down spin-orbitals are never linearly combined. In this way, as generators for a system with $n$ orbitals, we have a set of $\frac{n^2+n}{2}$ symmetric and $\frac{n^2-n}{2}$ antisymmetric matrices. 
To further reduce computational efforts, we do not consider mixing all orbitals with the same spin but we simply linearly combine orbitals with the same spin that possesses the same geometric symmetries.
One can see the optimization of orbitals as a mixing of the starting orbitals weighted by the rotation vector $\bm{R}$. Since the number of energy derivatives depends on the number of non-zero rotation parameters, it is considerably reduced  by taking into account the above-mentioned symmetries.
\\
{\it \textbf{Quantum mutual information matrix}}\\
To study the correlation present in our wave functions, VQE, WAHTOR-optimised or diagonalised ground states, we consider the quantum mutual information between the qubits that map the spin-orbitals of the system under consideration. The quantum mutual information between qubits $i$ and $j$ is defined as
\begin{equation}
I_{ij}=(S_i+S_j-S_{ij})\delta_{ij}
\end{equation}
where $S_{ij}$ and $S_j$ are, respectively, the one and two qubits Von Neumann entropy defined as follow
{\bf  qui non è chiarissimo. Io definirei separatemente Si e Sij altrimenti si perde il filo } 
\begin{equation}
S_{k}=-Tr(\rho_{k} log\rho_{k})
\end{equation}
Here $k$ is a set of one or two indices belonging to the set of all qubits $\Omega$ and $\rho_{k}$ is the reduced density matrix obtained from the density matrix $\rho$ tracing out over all the indices not belonging to $k$ 
\begin{equation}
\rho_{k}=Tr_{\{\Omega-k\}}(\rho)
\end{equation}
We represent the quantum mutual information as a symmetric matrix with elements along the diagonal equal to zero by definition, as done in \cite{Tkachenko2020}. The value of the correlation between the qubits can be observed in the upper or the lower triangular part of this matrix.

{\it \textbf{Orbital analysis}}\\
Here is described the $\delta$ parameter used to perform the orbital analysis....
